Stable Gaussian Process based Tracking Control of Lagrangian Systems

High performance tracking control can only be achieved if a good model of the dynamics is available. However, such a model is often difficult to obtain from first order physics only. In this paper, we develop a data-driven control law that ensures closed loop stability of Lagrangian systems. For this purpose, we use Gaussian Process regression for the feed-forward compensation of the unknown dynamics of the system. The gains of the feedback part are adapted based on the uncertainty of the learned model. Thus, the feedback gains are kept low as long as the learned model describes the true system sufficiently precisely. We show how to select a suitable gain adaption law that incorporates the uncertainty of the model to guarantee a globally bounded tracking error. A simulation with a robot manipulator demonstrates the efficacy of the proposed control law.

==> figure/const_gains.tex <==
\begin{tikzpicture}
\pgfplotsset{
  set layers,% using layers
  mark layer=axis tick labels% defines the layer of the marks
}
\begin{axis}[
  xlabel={$q_1$ [rad]},
  ylabel={$\dot{q}_1$ [rad/s]},
  line width=1pt,
  grid = major,
  height=5.5cm,
  width=\columnwidth,
  xmin=-1.3, xmax=1.2, ymin=-1.2, ymax=1.2]
\addplot[color=blue,style=loosely dashed,no marks, line width=1pt] table [x index=0,y index=1]{data/const_gains.dat};
\addplot+[color=red,no marks,style=loosely dotted, line width=1pt] table [x index=2,y index=3]{data/const_gains.dat};
\addplot+[mark=+,color=green!70!black, only marks,mark size=5, line width=1pt] table [x index=0,y index=1]{data/training_points.dat};
\end{axis}
\end{tikzpicture} 

==> figure/manipulator.tex <==

\newcommand{\nvar}[2]{%
    \newlength{#1}
    \setlength{#1}{#2}
}

% Define a few constants for drawing
\nvar{\dg}{0.3cm}
\def\dw{0.25}\def\dh{0.5}
\nvar{\ddx}{1.5cm}

% Define commands for links, joints and such
\def\link{\draw [double distance=1.5mm, very thick] (0,0)--}
\def\joint{%
    \filldraw [fill=white] (0,0) circle (5pt);
    \fill[black] circle (2pt);
}
\def\grip{%
    \draw[ultra thick](0cm,\dg)--(0cm,-\dg);
    \fill (0cm, 0.5\dg)+(0cm,1.5pt) -- +(0.6\dg,0cm) -- +(0pt,-1.5pt);
    \fill (0cm, -0.5\dg)+(0cm,1.5pt) -- +(0.6\dg,0cm) -- +(0pt,-1.5pt);
}
\def\robotbase{%
    \draw[rounded corners=8pt] (-\dw,-\dh)-- (-\dw, 0) --
        (0,\dh)--(\dw,0)--(\dw,-\dh);
    \draw (-0.5,-\dh)-- (0.5,-\dh);
    \fill[pattern=north east lines] (-0.5,-1) rectangle (0.5,-\dh);
}

% Draw an angle annotation
% Input:
%   #1 Angle
%   #2 Label
% Example:
%   \angann{30}{$\theta_1$}
\newcommand{\angann}[2]{%
    \begin{scope}[red]
    \draw [dashed, red] (0,0) -- (1.2\ddx,0pt);
    \draw [->, shorten >=3.5pt] (\ddx,0pt) arc (0:#1:\ddx);
    % Unfortunately automatic node placement on an arc is not supported yet.
    % We therefore have to compute an appropriate coordinate ourselves.
    \node at (#1/2-2:\ddx+8pt) {#2};
    \end{scope}
}

% Draw line annotation
% Input:
%   #1 Line offset (optional)
%   #2 Line angle
%   #3 Line length
%   #5 Line label
% Example:
%   \lineann[1]{30}{2}{$L_1$}
\newcommand{\lineann}[4][0.5]{%
    \begin{scope}[rotate=#2, blue,inner sep=2pt]
        \draw[dashed, blue!40] (0,0) -- +(0,#1)
            node [coordinate, near end] (a) {};
        \draw[dashed, blue!40] (#3,0) -- +(0,#1)
            node [coordinate, near end] (b) {};
        \draw[|<->|] (a) -- node[fill=white] {#4} (b);
    \end{scope}
}

% Draw mass annotation
% Input:
%   #1 mass label offset (optional)
%   #2 link angle
%   #3 link length
%   #4 mass label
% Example:
%   \massann[1]{30}{2}{$m_1$}
\newcommand{\massann}[4][0.4]{%
    \begin{scope}[rotate=#2, black,inner sep=2pt]
    	\filldraw [fill=black] (#3/2,0) circle (2pt);
    	\node[] at (#3/2,#1)  {#4};
    \end{scope}
}
% Define the kinematic parameters of the three link manipulator.
\def\thetaone{120}
\def\Lone{2}
\def\thetatwo{30}
\def\Ltwo{2}

\begin{tikzpicture}
    \robotbase
    \begin{scope}[shift=(0:0), rotate=-90]
    \angann{\thetaone}{$q_1$}
    \lineann[1.2]{\thetaone}{\Lone}{$l_1$}
    \link(\thetaone:\Lone);
    \joint
    \node[] at (0,-0.5)  {$\tau_1$};
    \begin{scope}[shift=(\thetaone:\Lone), rotate=\thetaone]
        \angann{\thetatwo}{$q_2$}
        \lineann[-1.5]{\thetatwo}{\Ltwo}{$l_2$}
        \link(\thetatwo:\Ltwo);
        \joint
        \node[] at (0,-0.5)  {$\tau_2$};
        \node[] at (-0.2,0.5)  {$m_1$};
        \begin{scope}[shift=(\thetatwo:\Ltwo), rotate=\thetatwo]
                \grip
                \node[] at (0,0.7)  {$m_2$};
        \end{scope}
    \end{scope}
    \end{scope}
    \draw[->] (\Lone,0) -- node[right] {$g$} (\Lone,-\dh);
\end{tikzpicture}


==> figure/training_bsb.tex <==
\begin{tikzpicture}[auto, node distance=3cm,>=latex']
\tikzstyle{block} = [draw, fill=white, rectangle, minimum height=2em, minimum width=1em]
\tikzstyle{sum} = [draw, fill=white, circle, node distance=1cm]
\tikzstyle{input} = [coordinate]
\tikzstyle{output} = [coordinate]
\tikzstyle{t_output} = []
\tikzstyle{pinstyle} = [pin edge={to-,thin,black}]

    \node [input, name=input] {};
    \node [block, right of=input,node distance=1.8cm] (controller) {$\scriptstyle \text{Controller}$};
    \node [block, right of=controller,node distance=1.9cm] (robot) {$\scriptstyle \text{System}$};
    \node [block, right of=robot,node distance=3.1cm] (hatrobot) {$\scriptstyle H(\q)\ddq+C(\q,\dq)\dq+\g(\q)$};
    
    \node [output, right of=hatrobot,node distance=1.7cm] (output) {};
    

	\draw [->] (input) -- node[name=t1] {$\scriptstyle \qd,\dqd,\ddqd$} (controller);
	\draw [->] (controller) -- node[name=t,below] {$\scriptstyle \bm\tau$} (robot);
    \draw [->] (robot) -- node[name=q] {$\scriptstyle \ddq,\dq,\q$} (hatrobot);
    \draw [-] (hatrobot) -- node[name=o,below, right=0.5mm] {$\scriptstyle \hat{\bm\tau}$} (output);
    
    \coordinate [below of=q,node distance=1.1cm] (dp) {};
    \node [t_output, right of=dp,node distance=1cm] (x_output) {$\scriptstyle\{X\}$};
    \node [t_output, above of=x_output,node distance=2.6cm] (y_output) {$\scriptstyle\{Y\}$};
    \draw [->] (q) |- (dp) -| (controller);
    
    
    \node [sum, above of=q,node distance=1cm,label={[label distance=0cm]20:-}] (sum) {};
    \node [output, above right of=sum,node distance=1cm] (output2) {\{Y\}};
    
    \draw [->] (dp) -- node[name=q1] {} (x_output);
    \draw [->] (sum) |- (y_output);
    
    \draw [->] (t) |- (sum);
    \draw [->] (output) |- (sum);

\end{tikzpicture}

==> figure/var_gains_values.tex <==
\begin{tikzpicture}
\pgfplotsset{
  set layers,% using layers
  mark layer=axis tick labels% defines the layer of the marks
}
\begin{axis}[
  ylabel={$\frac{\Verts{K_d}+\Verts{K_p}}{\Verts{K_{d,\text{static}}}+\Verts{K_{p,\text{static}}}}$},
  xlabel={$t$ [s]},
  height=4.5cm,
  width=\columnwidth,
  line width=1pt,
  grid = major,
  xmin=0, xmax=20, ymin=0.5, ymax=6]
\addplot[color=red,no marks, line width=1pt] table [x index=0,y index=1]{data/const_gains_values.dat};
\addplot+[mesh,point meta=\thisrowno{1}, no marks,line width=1pt, shader=interp] table [x index=0,y index=1]{data/var_gains_values.dat};
\legend{}
\end{axis}
\end{tikzpicture} 
